Robust Information Retrieval

Beyond effectiveness, the robustness of an information retrieval (IR) system is increasingly attracting attention. When deployed, a critical technology such as IR should not only deliver strong performance on average but also have the ability to handle a variety of exceptional situations. In recent years, research into the robustness of IR has seen significant growth, with numerous researchers offering extensive analyses and proposing myriad strategies to address robustness challenges. In this tutorial, we first provide background information covering the basics and a taxonomy of robustness in IR. Then, we examine adversarial robustness and out-of-distribution (OOD) robustness within IR-specific contexts, extensively reviewing recent progress in methods to enhance robustness. The tutorial concludes with a discussion on the robustness of IR in the context of large language models (LLMs), highlighting ongoing challenges and promising directions for future research. This tutorial aims to generate broader attention to robustness issues in IR, facilitate an understanding of the relevant literature, and lower the barrier to entry for interested researchers and practitioners.

==> Sections/presenters.tex <==
\vspace{-2mm}
\section{Presenters}
\vspace{-1mm}
\naming{Yu-An Liu} is a Ph.D. student at the Institute of Computing Technology, Chinese Academy of Sciences. 
He obtained his B.Eng. from Shandong University.
His research centers on information retrieval, with a particular focus on adversarial and out-of-distribution robustness of IR systems.
He is the first author of several full papers on adversarial robustness in IR, presented at SIGIR’23 \cite{liu2023topic}, CIKM’23 \cite{liu2023black}, AAAI’24 \cite{liu2024perturbation}, and SIGIR'24 \cite{liu2024multi}, as well as a paper on OOD robustness in IR at Gen-IR@SIGIR'23 \cite{liu2023robustness}.

\naming{Ruqing Zhang} is an Associate Researcher at the Institute of Computing Technology, Chinese Academy of Sciences. 
Her recent research focuses on information retrieval, with a particular emphasis on the robustness of information retrieval systems, trustworthy retrieval through the lens of causality, and generative information retrieval.
She has authored several papers in the field of robust information retrieval \cite{liu2023topic,liu2023robustness,liu2023black,liu2024perturbation,wu2022neural,wu2022prada,wu2022certified,liu2024multi}. 
Additionally, she was a co-organizer of tutorials and workshops at SIGIR, WWW, ECIR, and SIGIR-AP, e.g., Gen-IR workshops at SIGIR'23 and SIGIR'24, and Gen-IR tutorials at SIGIR-AP'23/WWW'24/ECIR'24.

\naming{Jiafeng Guo} is a Researcher at the Institute of Computing Technology, Chinese Academy of Sciences (CAS) and a Professor at the University of Chinese Academy of Sciences. 
He is the director of the CAS key lab of network data science and technology. 
He has worked on a number of topics related to Web search and data mining, with a current focus on neural models for information retrieval and natural language understanding. 
He has received multiple best paper (runner-up) awards at leading conferences (CIKM’11, SIGIR’12, CIKM’17, WSDM’22). 
He has been (co)chair for many conferences, e.g.,  reproducibility track co-chair of SIGIR'23, workshop co-chair of SIGIR'21, and short paper co-chair of SIGIR'20. 
He served as an associate editor for ACM Transactions on Information Systems and Information Retrieval Journal. 
Jiafeng has previously taught tutorials at many IR-related conferences.

\naming{Maarten de Rijke} is a Distinguished University Professor of Artificial Intelligence and Information Retrieval at the University of Amsterdam. 
His research is focused on designing and evaluating trustworthy technology to connect people to information, particularly search engines, recommender systems, and conversational assistants. 
He is the scientific director of the Innovation Center for Artificial Intelligence and a former editor-in-chief of ACM Transactions on Information Systems and of Foundations and Trends in Information Retrieval, and a current co-editor-in-chief of Springer’s Information Retrieval book series, (associate) editor for various journals and book series. 
He has been general (co)chair or program (co)chair for CIKM, ECIR, ICTIR, SIGIR, WSDM, WWW, and has previously taught tutorials at these same venues and AAAI.



